CFedAvg: Achieving Efficient Communication and Fast Convergence in Non-IID Federated Learning

Federated learning (FL) is a prevailing distributed learning paradigm, where a large number of workers jointly learn a model without sharing their training data. However, high communication costs could arise in FL due to large-scale (deep) learning models and bandwidth-constrained connections. In this paper, we introduce a communication-efficient algorithmic framework called CFedAvg for FL with non-i.i.d. datasets, which works with general (biased or unbiased) SNR-constrained compressors. We analyze the convergence rate of CFedAvg for non-convex functions with constant and decaying learning rates. The CFedAvg algorithm can achieve an $\mathcal{O}(1 / \sqrt{mKT} + 1 / T)$ convergence rate with a constant learning rate, implying a linear speedup for convergence as the number of workers increases, where $K$ is the number of local steps, $T$ is the number of total communication rounds, and $m$ is the total worker number. This matches the convergence rate of distributed/federated learning without compression, thus achieving high communication efficiency while not sacrificing learning accuracy in FL. Furthermore, we extend CFedAvg to cases with heterogeneous local steps, which allows different workers to perform a different number of local steps to better adapt to their own circumstances. The interesting observation in general is that the noise/variance introduced by compressors does not affect the overall convergence rate order for non-i.i.d. FL. We verify the effectiveness of our CFedAvg algorithm on three datasets with two gradient compression schemes of different compression ratios.

==> Supporting_Preambles/jackmac.tex <==
%>From snoeyink%cs.ubc.ca@cs.Technion.AC.IL Wed Nov  3 08:18:27 1993
%Received: from csmail.cs.technion.ac.il by math.tau.ac.il (5.67/math.tau-930921)
	%id AA17625; Wed, 3 Nov 93 08:18:23 +0200
%Received: from csc (csc.cs.technion.ac.il) by csmail.cs.Technion.AC.IL (4.1/3.14)
	%id AA14244; Wed, 3 Nov 93 01:19:10 IST
%Received: from csa by csc (4.1/3.14)
	%id AA24688; Wed, 3 Nov 93 01:19:48 IST
%Received: from grolsch.cs.ubc.ca by csa (4.1/3.14)
	%id AA20525; Wed, 3 Nov 93 01:11:28 IST
%Return-Path: <snoeyink@cs.ubc.ca>
%Received: from cascade.cs.ubc.ca by grolsch.cs.ubc.ca with SMTP id AA13516
  %(5.65c/IDA-1.3.5 for alon@cs.Technion.AC.IL); Tue, 2 Nov 1993 13:56:34 -0800
%Date: Tue, 2 Nov 1993 13:56:34 -0800
%From: Jack Snoeyink <snoeyink%cs.ubc.ca@cs.Technion.AC.IL>
%Message-Id: <199311022156.AA13516@grolsch.cs.ubc.ca>
%Received: by cascade.cs.ubc.ca (4.1/SMI-4.1)
	%id AA21873; Tue, 2 Nov 93 13:56:33 PST
%To: alon@cs.Technion.AC.IL
%In-Reply-To: Alon Efrat's message of Sun, 31 Oct 93 23:38:48 IST <9310312138.AA19880@csc>
%Subject: LaTex Macros
%Status: RO
%Content-Length: 19065
%X-Lines: 638
%
%
%I'm in oberwolfach w/ micha, so I';ll just send you this and answer
%your questions on it when I get back to vancouver next week...
%
    %o                                    Jack
  %_/\_.
%(')>-(`)                          snoeyink@cs.ubc.ca
%----figbox.tex----

% 12 Oct 90 LaTeX figure boxing macros  by Jack Snoeyink
%					w/ ideas from John Hershberger
%					and code from Tom Rokicki
%%%%%%%%%%%%%%%%%
% 
% This file contains two classes of macros for dealing with figures in
% Latex documents:  
%  \figbox (and its relatives) take a box containing a figure or table
%    or whatever, caption it, and either place it on the page and wrap the
%    text around it or let it float (as usual).
%  \boxeps and \boxps take encasulated or plain postscript from a file
%    and put it in a box for use by \figbox
%
%%%%%%%%%%%%%%%%
%
% The most important macro for dealing with boxes is:
%
% \figbox: caption a box as a figure or table and place it in the margin
% 	(a marginal box) or float it (a floating box).
% 	Wide marginal boxes are promoted to one column floats; wide one
% 	column floats are promoted to two column floats.
%
% Usage: \figbox [*htblr] {box} {style} {label} {caption}
%
% The optional argument default is [htb].  Other choices
%   * two column (must come first),
%   h here, t top, b bottom (as in latex),
%   l left, r right (marginal boxes that do not float)
%
% NB: Left and right marginal boxes will not overlap in height.
%
% Two column figures default to htb unless some other 
%   	options follow the *.
%   They can also be specified by style {figure*} or {table*}.
%
% box is a box containing a figure or table.
% style is the caption style {figure}, {figure*}, {table}, or {table*}.  
% label is the label assigned.
%	if empty, the figure will not be labeled.
% caption is of the form {}, {Caption} or {[short caption] Long caption},
%       where the short caption goes into the list of figures/tables.
%	if empty, the figure will not be captioned or labeled.
% 
% The lower level macro \captionbox, described much later, can be used
% to combine two or more captioned figures into a single marginal or
% floating box.
%
%%%%%%%%%%%%%%%%
%
% options defined by macros are: \captionstyle \boxcaptionstyle
% \maxfigfraction \figboxhang \figboxmargin 
%
% \captionstyle is executed for all floating box captions
% \boxcaptionstyle is executed for all marginal box captions.
%	Default \raggedright
% \maxfigfraction is the maximum fraction of a column that can be taken up
% 	by a marginal box before it gets converted to a float.
% 	Default .6
% dimen \figboxhang is the distance a marginal box hangs into the margin.
%	Default 0pt
% dimen \figboxmargin is the width of space between the text and a
% 	marginal box. 
%	Default .15in
%
%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%
%
% The most important macros for turning postscript into boxes are:
% 
% \boxeps: Form a box containing encapsulated postscript from a file at a
%	given scale.
% \boxps: Form a box containing postscript from a file at a given scale, 
% 	width, and height.
% 
%
% Usage: \boxeps[local commands] {file} {scale}
%	 \boxps[local commands] {file} {scale} {width} {height}
%
% The optional local commands are executed after scaling. As described
% 	below, they are useful for setting origins, non-uniform scaling, etc?
% file is the filename in the \figuredirectory and without the .ps
% 	extension.
% scale is a real number: 1 to use the drawn size.  0.9 to use 90% of
% 	drawn size.  Can be changed by local commands. (see below)
% width and height are dimensions of the box produced by \boxps.
%
%%%%%%%%%%%%%%%%
%
% options: \DVIscaling \figuredirectory \missingfigure \boxer
% local commands: \horizscale \vertscale
%
% \DVIscaling is the number the dvi to ps converter considers a unit
% 	scaling transformation.  Default: 1 for dvi2ps  --- 100 for
% 	some of Rokicki's versions of dvips.
%
% \globalscaling is the scaling applied to every picture --- useful
% 	for making double size figures for journals.  Default: 1
%
% \figuredirectory is the pathname where figure postscript files are kept.
%	Default: ./figure
%
% \missingfigure{file} is executed when the file is not found.
%	Default: \def\missingfigure#1{\hbox{Missing figure #1.ps}}
%
% \boxer is the command used by \boxps to make a box of the desired size
% 	containing the figure.  Possible commands depend on the origin of
% 	the figure, and include \llboxer \lcboxer \ulboxer and \ccboxer.
% 	(ll = lower left, ul = upper left, cc = dead center, etc.)
%	\boxer can be defined in the local commands or globally.
%
% Local commands \horizscale, and \vertscale can scale the picture
% 	horizontally and vertically by different factors.  \scale
% 	scales the picture uniformly.  Scales accumulate.
%
%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%
%
% Default options
%

\def\captionstyle{}
\def\boxcaptionstyle{\raggedright}

\def\maxfigfraction{.6}% 	--- max frac of column for marg figure

\newdimen\figboxmargin%		--- margin between text and picture
\figboxmargin = .15in

\newdimen\figboxhang%		--- amount to hang picture into margin
\figboxhang = 0pt

\def\DVIscaling{1}%		--- for dvi2ps
\def\globalscaling{1}%		--- for scaling everything
\def\figuredirectory{./figures}%--- where to find the .ps files 
\let\boxer=\llboxer%		--- default origin in lower left for non-
%				      encapsulated postscript figures

\def\missingfigure#1{\hbox{Missing figure #1.ps}}


%%%%%%%%%%%%%%%%
%
% Use latex internals
%
\catcode `\@=11
\special{! /@scaleunit 1 def }

\newbox\figurebox

\def\figbox{%	[place] box style label caption
\@ifnextchar[{\figboxaux}{\figboxaux[htb]}}

%
% Parse position parameters and try appropriate placement
%
\long\def\figboxaux[#1#2]#3#4#5#6{%	--- want left margin figure?
\writepict{{#3}{#4}{#5}{#6}}%		--- save figure if journalpicts
\setbox\figurebox\hbox{#3}%
\if l#1\tryleftbox{#4}{#5}{#6}%
\else%					--- want right margin figure?
\if r#1\tryrightbox{#4}{#5}{#6}%
\else%					--- want one or two column figure?
\if *#1\checktwocoloptions#2]{\box\figurebox}{#4*}{#5}{#6}%
\else\tryonecol[#1#2]{#4}{#5}{#6}%
\fi
\fi
\fi\ignorespaces}

%
% Try a placement; promote if too wide
%

\long\def\tryleftbox#1#2#3{%		--- does left margin figure fit?
\ifdim\wd\figurebox>\maxfigfraction\columnwidth \tryonecol[htb]{#1}{#2}{#3}%
\else\leftbox{\captionbox{\box\figurebox}{#1}{#2}{#3}}\fi}

\long\def\tryrightbox#1#2#3{%	--- does right margin figure fit?
\ifdim\wd\figurebox>\maxfigfraction\columnwidth \tryonecol[htb]{#1}{#2}{#3}%
\else\rightbox{\captionbox{\box\figurebox}{#1}{#2}{#3}}\fi}

\def\checktwocoloptions{%	--- make sure twocol has htb or p
\@ifnextchar]{\floatbox[htb}{\floatbox[}}

\long\def\tryonecol[#1]#2#3#4{%	--- does one column figure fit?
\ifdim\wd\figurebox>\columnwidth \floatbox[#1]{\box\figurebox}{#2*}{#3}{#4}%
\else\floatbox[#1]{\box\figurebox}{#2}{#3}{#4}\fi}

%
% Do the work for a floating box.
%
% \floatbox[place]{box} {style} {label} {caption}
%

\long\def\floatbox[#1]#2#3#4#5{%
\begin{#3}[#1]
\hbox to \hsize{\hfil#2\hfil}
\captionandlabel{#3}{#4}{#5}
\end{#3}
}


%
% Make a caption the width of the box with given style. 
%
%\captionbox {box} {style} {label} {[optshortcap] caption}
%
% options: \boxcaptionstyle 
%
%%%%%%%%%%%%%%%%
%
% This can be used with box commands (\hbox, \vbox, \mbox, and the like),
% along with \figbox with an empty caption, to place two or more captioned
% boxes in a single marginal or floating box.   
%
% e.g. \figbox{\hbox{
%		     \captionbox{ \boxeps{fig1}1} {figure} {f1} {a figure}
%		     \hskip 1in
%		     \captionbox{ \boxeps{tab1}1} {table} {t1} {a table}
%		    }} {figure} {ignored-label} {}
%

\long\def\captionbox#1#2#3#4{% box style label {[optshortcap] caption}
\setbox\figurebox\hbox{#1}%
\parbox[t]{\wd\figurebox}{%
\bigskip\box\figurebox
\let\captionstyle=\boxcaptionstyle
\captionandlabel{#2}{#3}{#4}
\bigskip
}}

%				--- caption and label if label is nonempty
\def\captionandlabel#1#2#3{% 	--- {style} {label} {caption}
\def\testit{#3}%
\ifx\testit\empty\else%		--- if non empty caption
\writecapt{{#1}{#2}{#3}}%	--- save for journal figs
\captypeunstarred#1*.%		--- remove optional stars
\getcaption#3\endc@ption%       --- parse the caption
\def\testit{#2}%		--- check for empty label
\ifx\testit\empty\else\label{#2}\fi
\fi}

\def\captypeunstarred#1*#2.{%	--- remove two-column star from style
\def\@captype{#1}}

%
% Parse the caption of the form {caption} or {[short] long caption} 
%

\def\getcaption{\@ifnextchar[{\getcaptwo}{\getcapone}}
\long\def\getcapone#1\endc@ption{\caption[#1]%
{\def\baselinestretch{1}\Large\normalsize\captionstyle\ignorespaces #1}}
\long\def\getcaptwo[#1]#2\endc@ption{\caption[#1]%
{\def\baselinestretch{1}\Large\normalsize\captionstyle\ignorespaces #2}}

%
% Do the right thing with an already captioned marginal box
%
% \leftbox{box}
% \rightbox{box}
%
% options: \figboxmargin \figboxhang \figuredirectory

\newdimen\figboxht
\newcount\figboxn


\newcount\figboxlines%		--- picture height in number of lines
\newdimen\figboxwid%		--- picture width

\newif\ifisleftbox

\long\def\leftbox#1{%
\setbox\figurebox\hbox{#1}\global\isleftboxtrue
\startmarginbox
\vadjust{\smash{\rlap{\hskip\hsize\hskip\figboxhang
\llap{\raise.7\baselineskip\box\figurebox\hskip\rightskip}}}}%
\endmarginbox%
}

\long\def\rightbox#1{%
\setbox\figurebox\hbox{#1}\global\isleftboxfalse
\startmarginbox
\smash{\llap{\raise.7\baselineskip\box\figurebox\hskip\figboxmargin}}%
\endmarginbox%
}

\def\startmarginbox{%
\ifvmode\passpict\let\endmarginbox=\indent
\else\message{WARNING: marginbox in not in vmode}\hfilneg\ \passpict
\let\endmarginbox=\relax\fi
%
\figboxht=\dp\figurebox%	 actual height
\advance\figboxht by 1.3\baselineskip% round up
\vskip\figboxht\penalty-300\vskip-\figboxht% filbreak trick
\divide\figboxht by\baselineskip%      how many lines?
\global\figboxlines=\figboxht
%
\global\figboxwid=\wd\figurebox
\global\advance\figboxwid by \figboxmargin
\global\advance\figboxwid by -\figboxhang
\setmypar\noindent}
%

%
% Useful macros
%
% for lengthening (and shortening) picture space
%
\def\addlines#1{\global\advance\figboxlines by #1\myparshape}
\def\zerolines{\origpar\global\figboxlines=0\myparshape}

%
% for passing any marginal figures
%
\def\passpict{\par\ifnum\figboxlines>1\vskip\figboxlines\baselineskip
\zerolines\fi}

\def\emptybox#1#2{\hbox to #1{\vbox to #2{\vss}\hss}}

%%%%%%%%%%%%%%%%%%%%%
%\par hacking  
% We define our own version of Tex's \par and tell Latex it is the original

\global\let\origpar=\@@par%	--- Latex's saved version of Tex's \par
\global\let\dopar=\origpar
\global\def\@@par{\dopar}
\@setpar{\dopar}

\def\setmypar{\global\let\dopar=\mypar
\global\prevgraf=0\myparshape}

\def\mypar{\origpar\global\advance\figboxlines by -\prevgraf%
\global\prevgraf=0\myparshape}

\def\myparshape{\relax%
\ifnum\figboxlines>1\theparshape \else
\global\hangindent=0pt\global\hangafter=1%  these sometimes get restored...
\global\let\dopar=\origpar\fi}

\def\theparshape{%
\ifisleftbox\global\hangindent=-\figboxwid 
\else\global\hangindent=\figboxwid \fi
\global\hangafter=-\figboxlines \global\advance\hangafter by 1%
}


%%%%%%%%%%%%%%%%
%
%  Macros to make the list of figures and captions used by journals
%
%  To use, execute \journalpicts{scalefactor} at the beginning of the
%  file.  All figbox figures and tables will be written to a .pic file
%  and all captions to a .cap file.  On \enddocument, these files are
%  read in and the lists of figures and captions are produced.
%  
%  For non-english versions, or to add other types of floats, the
%  macro \definefnum should be changed.
%

\def\definefnum#1{%		--- ugly latex hacking to get the
%		 			right figure/table name 
\def\fnum@figure{Figure \ref{#1}}%
\def\fnum@table{Table \ref{#1}}%
\def\fnum@code{Algorithm \ref{#1}}%
}

\def\writepict#1{}
\def\writecapt#1{}

%%%%%%%%%%%%%%%%
% \journalpicts{globalscalefactor} writes all pictures and captions to
% 	files and modifies \enddocument to read these files and
% 	produce lists of enlarged figures and of captions
% 

\def\journalpicts#1{% 		global scale factor
\newwrite\pictfile
\newwrite\captfile
%
\openout\pictfile\jobname.pic
\openout\captfile\jobname.cap
%
\gdef\writepict##1{\unexpandedwrite\pictfile{\doit##1}}%
\gdef\writecapt##1{\unexpandedwrite\captfile{\doit##1}}%
%
\global\let\ENDdocument=\enddocument
\gdef\enddocument{\DOjournalpicts{#1}\ENDdocument}
}

%
%	generate enlarged figures 1 per page and list captions
%
\def\DOjournalpicts#1{{%
\def\writepict##1{}\closeout\pictfile
\def\writecapt##1{}\closeout\captfile
\@fileswfalse%			--- turn off toc, lof, and so on.
%
\onecolumn
\def\globalscaling{#1}
\def\doit##1##2##3##4{%		--- print a picture on blank page
%					{box}{style}{label}{caption}
\figboxaux[t]{\hss##1\hss}{##2}{}{}%
\vspace*{1in}
\definefnum{##3}%		--- use Figure \ref{label} or Table \ref{label}
\captionandlabel{##2}{}{##4}
\clearpage}%
%
\input\jobname.pic
%
\def\doit##1##2##3{%		--- print caption
%					{style}{label}{caption}
\definefnum{##2}%		--- use Figure \ref{label} or Table \ref{label}
\captionandlabel{##1}{}{##3}}%
%
\raggedright\let\captionstyle=\raggedright
\def\@makecaption##1##2{##1: ##2\par}%  --- Be sure captions aren't centered
%
\input\jobname.cap
}}%				--- to be followed by \enddocument



%%%%%%%%%%%%%%%%
%
%  Box macros
%
%%%%%%%%%%%%%%%%
%
% \boxeps[local commands] {file} {scale}
%
% options \DVIscaling \figuredirectory \scale \horizscale \vertscale
% \missingfigure \globalscaling
%
% \boxps[local commands] {file} {scale} {width} {height}
%
% \scale \horizscale \vertscale 

%
%  Various `boxers' --- which one is used depends on where the origin
%  of the picture is.  If you are using the bounding boxes of
%  encapsulated postscript, just use the default \llboxer.  Otherwise,
%  you have to figure out where the origin is and set \boxer appropriately.
%

\def\llboxer#1{\vbox to \figboxht{\vfil\hbox to \figboxwid{#1\hfill}}}
\def\lcboxer#1{\vbox to \figboxht{\vfil\hbox to \figboxwid{\hfill#1\hfill}}}
\def\oldboxer#1{\vbox to \figboxht{\vfil
		      \hbox to \figboxwid{\hfill\llap{#1\hskip4.25in}\hfill}}}
\def\ulboxer#1{\vbox to \figboxht{\hbox to \figboxwid{#1\hfill}\vfil}}
\def\ccboxer#1{\vbox to \figboxht{\vfil
			\hbox to \figboxwid{\hfill#1\hfill}\vfil}}

% a macro to strip the pt off a dimension
%
{\catcode`\p=12\catcode`\t=12
\gdef\removedimen#1pt{#1}}

\def\defscaled#1#2{#2=\DVIscaling#2%
\xdef#1{\expandafter\removedimen\the#2}}

\def\DVIspace{ }
\newdimen\hscalefactor
\newdimen\vscalefactor

\def\scale#1{\horizscale{#1}\vertscale{#1}}
\def\horizscale#1{\hscalefactor=#1\hscalefactor\figboxht=#1\figboxht}
\def\vertscale#1{\vscalefactor=#1\vscalefactor\figboxwid=#1\figboxwid}

%%%%%%%%%%%%%%%%
%

\def\boxps{%
\@ifnextchar[{\boxpsaux}{\boxpsaux[\relax]}}

\def\boxpsaux[#1]#2#3#4#5{%
{\figboxwid#4\figboxht#5\hscalefactor=1pt\vscalefactor=1pt%
\scale{#3}%
\scale{\globalscaling}%
#1%
\defscaled\DVIhscale\hscalefactor
\defscaled\DVIvscale\vscalefactor
\boxer{\special{psfile=\figuredirectory/#2.ps \DVIspace
		hscale=\DVIhscale\DVIspace 
		vscale=\DVIvscale}}}%
}


%%%%%%%%%%%%%%%%
% The following is from tex/inputs/epsf.tex by Tom Rokicki
% with slight modifications by Jack Snoeyink.
%
%   Written by Tomas Rokicki of Radical Eye Software, 29 Mar 1989.
%
%   Include an ecapsulated postscript graphic.
%   Works by finding the bounding box comment.
%
\newread\Epsffilein
\newif\ifEpsffileok
\newif\ifEpsfbbfound

\newdimen\pspoints
\pspoints=1in
\divide\pspoints by 72


\def\boxeps{%
\@ifnextchar[{\boxepsaux}{\boxepsaux[\relax]}}
\def\boxepsaux[#1]#2#3{%
%
%   The first thing we need to do is to open the
%   PostScript file, if possible.
%
\openin\Epsffilein=\figuredirectory/#2.ps 
\ifeof\Epsffilein\message{I couldn't open \figuredirectory/#2.ps }%
\missingfigure{#2}
\else
%
%   Okay, we got it.  Now we scan lines until we find one
%   that doesn't start with a percentage sign.  We're
%   looking for the bounding box comment.
%
   {\Epsffileoktrue\Epsfbbfoundfalse
    \catcode`\%=11 \catcode`\\=11
    \catcode`\{=11 \catcode`\}=11
    \catcode`\$=11 \catcode`\^=11
    \catcode`\&=11 \catcode`\#=11
    \catcode`\~=11 \catcode`\_=11
    \loop
       \read\Epsffilein to \Epsffileline
       \ifeof\Epsffilein\Epsffileokfalse\else
%
%   Now we check to make sure the first character is a % sign,
%   and that the rest are `%BoundingBox:' if necessary.
%
          \expandafter\Epsfaux\Epsffileline . .\\%
       \fi
   \ifEpsffileok\repeat
   \ifEpsfbbfound
	\figboxht=\Epsfury\pspoints
	\advance\figboxht by-\Epsflly\pspoints
	\figboxwid=\Epsfurx\pspoints
	\advance\figboxwid by-\Epsfllx\pspoints
   \else
	\message{No bounding box comment in \figuredirectory/#2.ps }%
	\figboxwid=2in\figboxht=1in%
   \fi%
   \immediate\closein\Epsffilein
   \hscalefactor=1pt\vscalefactor=1pt%
   \scale{#3}%
   \scale{\globalscaling}%
   #1%
%
   \defscaled\DVIhscale\hscalefactor
   \defscaled\DVIvscale\vscalefactor
%
   \hscalefactor=-\Epsfllx\hscalefactor
   \hscalefactor=1.00375\hscalefactor%	--- 72.27/72 = TeXpoints/PSpoints
   \defscaled\DVIhoffset\hscalefactor
%
   \vscalefactor=-\Epsflly\vscalefactor
   \vscalefactor=1.00375\vscalefactor%	--- 72.27/72 = TeXpoints/PSpoints
   \defscaled\DVIvoffset\vscalefactor
%
   \llboxer{\special{psfile=\figuredirectory/#2.ps \DVIspace
		hoffset=\DVIhoffset\DVIspace
		voffset=\DVIvoffset\DVIspace
                hscale=\DVIhscale\DVIspace 
                vscale=\DVIvscale}} }%
\fi
}%
%
%   We need these for comparison purposes.
%
{\catcode`\%=11 \global\let\Epsfpar=\par
\global\let\Epsfpercent=%\global\def\Epsfbblit{%BoundingBox:}}%
%
%   This is our function that checks for `%BoundingBox:' and grabs the
%   values if they are found.
%
\long\def\Epsfaux#1#2 #3\\{\relax\ifx#1\Epsfpercent
   \def\testit{#2}\ifx\testit\Epsfbblit
      \Epsfsize #3 . . . .\\%
      \global\Epsffileokfalse
      \global\Epsfbbfoundtrue
   \fi\else\ifx#1\Epsfpar\else\global\Epsffileokfalse\fi\fi}%
%
%   Here we grab the values and stuff them in the appropriate definitions.
%
\def\Epsfsize#1 #2 #3 #4 #5\\{\global\def\Epsfllx{#1}\global\def\Epsflly{#2}%
   \global\def\Epsfurx{#3}\global\def\Epsfury{#4}}%




\catcode`\@=12 			% done with with internals

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% For backward compatability
%
% \pic file; height in inches; width in inches; caption\par
% \picsc file; ht (in); wid (in); scale; caption\par
%
% \mpic file; height in inches; width in inches; caption\par
% \mpicsc file; ht (in); wid (in); scale; caption\par
%
%%%%%%%%%%%%%%%%

\def\pic#1;#2;#3;#4\par{\picsc#1;#2;#3;1;#4\par}% file; wd; ht; caption 

\def\picsc#1;#2;#3;#4;#5\par{% file; wd; ht; scale; caption
\figbox[htb]{\boxeps{#1}{#4}%{#2in}{#3in}%
}{figure}{#1}{%
% (#1: #2x#3 sc #4) % 			Uncomment for debugging
#5}}


\def\mpic#1;#2;#3;#4\par{\mpicsc#1;#2;#3;1;#4\par}% file; wd; ht; caption 

\def\mpicsc#1;#2;#3;#4;#5\par{% file; wd; ht; scale; caption
\figbox[l]{\boxeps{#1}{#4}%{#2in}{#3in}%
}{figure}{#1}{%
% (#1: #2x#3 sc #4) % 			Uncomment for debugging
#5}}




